Silicon Quantum Electronics

This review describes recent groundbreaking results in Si, Si/SiGe and dopant-based quantum dots, and it highlights the remarkable advances in Si-based quantum physics that have occurred in the past few years. This progress has been possible thanks to materials development for both Si quantum devices, and thanks to the physical understanding of quantum effects in silicon. Recent critical steps include the isolation of single electrons, the observation of spin blockade and single-shot read-out of individual electron spins in both dopants and gated quantum dots in Si. Each of these results has come with physics that was not anticipated from previous work in other material systems. These advances underline the significant progress towards the realization of spin quantum bits in a material with a long spin coherence time, crucial for quantum computation and spintronics.

==> outlook-FZ.tex <==
\section{Outlook}\label{outlook}

Here we describe the outlook\\

%\subsection{Single-shot readout of an electron spin}
%
%text


%\subsubsection{subsubsection1} - use if required

%\subsubsection{subsubsection2}



\section*{Acknowledgments}
FAZ, AM, ASD, MYS, LCLH and SR acknowledge support from the Australian Research Council Centre of Excellence for Quantum Computation and Communication Technology (project number CE110001029) and the US National Security Agency and the US Army Research Office under contract number W911NF-08-1-0527. GK acknowledges the technical support by Zhengping Jiang in the preparation of the NEMO figures and editorial aspects.  Gk also acknowledges the long time collaborations with Dr. Timothy b Boykin and his former student Dr. Neerav Kharche.  nanoHUB.org computational resources operated by the network for computational nanotechnology funded by the national science foundation have been used in this work.

